On the role of Lip Articulation in Visual Speech Perception

Generating realistic lip motion from audio to simulate speech production is critical for driving natural character animation. Previous research has shown that traditional metrics used to optimize and assess models for generating lip motion from speech are not a good indicator of subjective opinion of animation quality. Devising metrics that align with subjective opinion first requires understanding what impacts human perception of quality. In this work, we focus on the degree of articulation and run a series of experiments to study how articulation strength impacts human perception of lip motion accompanying speech. Specifically, we study how increasing under-articulated (dampened) and over-articulated (exaggerated) lip motion affects human perception of quality. We examine the impact of articulation strength on human perception when considering only lip motion, where viewers are presented with talking faces represented by landmarks, and in the context of embodied characters, where viewers are presented with photo-realistic videos. Our results show that viewers prefer over-articulated lip motion consistently more than under-articulated lip motion and that this preference generalizes across different speakers and embodiments.

==> table_1.tex <==
\begin{table}[t]
\caption{Perceptual score prediction performance. We report the performance of predicting the mean perceptual score from the sequence of augmented landmarks alone and from both the augmented and reference sequences as described in Section \ref{subsec_building_models_setup}. Statistical prior baseline always predicts the mean score computed on the training set. We report the means and the standard deviations on the test set from $100$ runs.}
  \label{tab:perceptual_results}
  \centering
  \begin{tabular}{lcc}
    \toprule
    % \textbf{Setup} & \textbf{MAE} & $\mathbf{\rho}$ \\
    \textbf{Setup} & \textbf{MAE} & $\rho$ \\
    \midrule
    Statistical Prior       & $0.73$ $(\pm 0.02)$ & $-$ \\
    Augmented Only          & $0.47$ $(\pm0.06)$ & $0.76$ $(\pm0.04)$ \\
    Augmented \& Reference  & $0.47$ $(\pm0.09)$ & $0.79$ $(\pm0.03)$\\
    \bottomrule
  \end{tabular}
\end{table}

